Elliot: a Comprehensive and Rigorous Framework for Reproducible Recommender Systems Evaluation

Recommender Systems have shown to be an effective way to alleviate the over-choice problem and provide accurate and tailored recommendations. However, the impressive number of proposed recommendation algorithms, splitting strategies, evaluation protocols, metrics, and tasks, has made rigorous experimental evaluation particularly challenging. Puzzled and frustrated by the continuous recreation of appropriate evaluation benchmarks, experimental pipelines, hyperparameter optimization, and evaluation procedures, we have developed an exhaustive framework to address such needs. Elliot is a comprehensive recommendation framework that aims to run and reproduce an entire experimental pipeline by processing a simple configuration file. The framework loads, filters, and splits the data considering a vast set of strategies (13 splitting methods and 8 filtering approaches, from temporal training-test splitting to nested K-folds Cross-Validation). Elliot optimizes hyperparameters (51 strategies) for several recommendation algorithms (50), selects the best models, compares them with the baselines providing intra-model statistics, computes metrics (36) spanning from accuracy to beyond-accuracy, bias, and fairness, and conducts statistical analysis (Wilcoxon and Paired t-test). The aim is to provide the researchers with a tool to ease (and make them reproducible) all the experimental evaluation phases, from data reading to results collection. Elliot is available on GitHub (https://github.com/sisinflab/elliot).

==> tables/backup_unique_table.tex <==

\begin{table*}[tbp]
\caption{Hold-out (HO), Cross-validation (CV)}
\small
%\begin{center}
%\resizebox{\textwidth}{!}{%
{
\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{0.29em}
\rowcolors{21}{white}{gray!15}
\begin{tabularx}{\textwidth}{X@{\hskip 0.8em}llllllllllllllllllr@{\hskip 0.8em}llllllllr@{\hskip 0.8em}llllllllr}

\hlineB{2.5}
\myrowcolour
 \multicolumn{ 38}{c}{\textbf{PRE-ELABORATION AND MODEL OPTIMIZATION STRATEGIES}} \\

\toprule

 & \multicolumn{ 19}{c}{\textbf{Splitting}}
 & \multicolumn{ 9}{c}{\textbf{Filtering}}
 & \multicolumn{ 9}{c}{\multirow{1}{*}{\textbf{Hyperparam.} \textbf{Tuning} }} 
\\
 \cmidrule(r){2-20}\cmidrule(lr){21-29}\cmidrule(l){30-38}


 & \multicolumn{ 7}{c}{Temporal} 
 & \multicolumn{ 10}{c}{Random} 
 & \multicolumn{ 1}{c}{\multirow{2}{*}{Fix}} 
 & \multicolumn{ 1}{c}{} 
 & \multicolumn{ 3}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Rating \\ Thld. \end{tabular}}} 
 & \multicolumn{ 5}{c}{\multirow{2}{*}{$k$-core}} 
 & \multicolumn{1}{l}{} 
 & \multicolumn{ 4}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Search \\ Strategy\end{tabular}}}
 & \multicolumn{ 4}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Search \\\ Space\end{tabular}}}
  & \multicolumn{1}{l}{}
 \\
 \cmidrule(r){2-8}\cmidrule(lr){9-18}

 
 & \multicolumn{ 2}{c}{\textit{Fix}} 
 & \multicolumn{ 5}{c}{\textit{HO}} 
 & \multicolumn{ 5}{c}{\textit{HO}} 
 & \multicolumn{ 3}{c}{$K$\textit{-HO}} 
 & \multicolumn{ 2}{c}{\textit{CV}} 
 & \multicolumn{ 1}{l}{} 
 & \multicolumn{ 1}{l}{} 
 & \multicolumn{ 3}{l}{} 
 & \multicolumn{ 5}{l}{} 
%  & \multicolumn{1}{l}{} 
%  & \multicolumn{ 4}{c}{Search Strategy}
%  & \multicolumn{ 4}{c}{Search Space} 
%  & \multicolumn{1}{l}{} 
 \\ 
  \cmidrule(r){2-3}\cmidrule(lr){4-8}\cmidrule(lr){9-13} \cmidrule(lr){14-16}\cmidrule(lr){17-18} \cmidrule{19-19} 
  \cmidrule(r){21-23}  \cmidrule(l){24-28}    \cmidrule(r){30-33} \cmidrule(l){34-37}

 
 & \rotatebox{90}{Best Tstp.} 
 & \rotatebox{90}{Handcrafted}
 & \rotatebox{90}{By-Ratio Sys.}
 & \rotatebox{90}{By-Ratio User}
 & \rotatebox{90}{Leave-$1$-out}
 & \rotatebox{90}{Leave-$n$-in}
 & \rotatebox{90}{Leave-$n$-out}
 & \rotatebox{90}{By-Ratio Sys.}
 & \rotatebox{90}{By-Ratio User}
 & \rotatebox{90}{Leave-$1$-out}
 & \rotatebox{90}{Leave-$n$-in}
 & \rotatebox{90}{Leave-$n$-out}
 & \rotatebox{90}{By-Ratio Sys.}
 & \rotatebox{90}{Leave-$1$-out}
 & \rotatebox{90}{Leave-$n$-out}
 & \rotatebox{90}{$k$-folds Sys.}
 & \rotatebox{90}{$k$-folds User}
 & \multicolumn{1}{c}{\rotatebox{90}{Computed}}
 & \rotatebox{90}{\textbf{Tot.}} 
 
 & \rotatebox{90}{Numerical}
 & \rotatebox{90}{Distributional}
 & \rotatebox{90}{User-Based}
%   & \rotatebox{90}{$k\text{-core}_\textit{User}$}
%  & \rotatebox{90}{$k\text{-core}_\textit{Item}$}
%  & \rotatebox{90}{Iterative $k$-core}
%  & \rotatebox{90}{$n$ rounds $k$-core}
  & \rotatebox{90}{User}
 & \rotatebox{90}{Item}
 & \rotatebox{90}{Iterative}
 & \rotatebox{90}{$n$-rounds}
 & \multicolumn{1}{c}{\rotatebox{90}{cold users}}
 
 & \rotatebox{90}{\textbf{Tot.}}
 & \rotatebox{90}{Grid}
 & \rotatebox{90}{Annealing}
 & \rotatebox{90}{Bayesian} 
 & \rotatebox{90}{Random}
 & \rotatebox{90}{Choice}
 & \rotatebox{90}{Uniform}
 & \rotatebox{90}{Normal}
 & \multicolumn{1}{c}{\rotatebox{90}{Log-Uniform}}
 & \rotatebox{90}{\textbf{Tot.}}
 
\\ 
\toprule


LensKit Java~\cite{DBLP:conf/recsys/EkstrandLKR11}    &  &  &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  &  & \checkmark & \checkmark & 10 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
Mymedialite~\cite{DBLP:conf/recsys/GantnerRFS11}   &  &  & \checkmark & \checkmark &  &  & \checkmark & \checkmark &  &  &  &  &  &  &  & \checkmark &  & \checkmark & 6 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
RankSys~\cite{DBLP:conf/sigir/Vargas14}       &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & 1 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
LibRec~\cite{DBLP:conf/um/GuoZSY15}         &  &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark &  & \checkmark &  & \checkmark & 11 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
Implicit\footnote{\url{https://github.com/benfred/implicit}}    &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & 1 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
OpenRec~\cite{DBLP:conf/wsdm/YangBGHE18}        &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & 1 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
RecQ~\cite{DBLP:conf/icdm/Yu0YLGW19} &  &  &  &  &  &  &  &  & \checkmark &  &  &  & \checkmark &  &  &  &  & \checkmark & 3 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
DeepRec~\cite{DBLP:conf/isca/GuptaHSWRWL0W20} &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  & \checkmark & 2 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
LensKit Python~\cite{DBLP:conf/cikm/Ekstrand20}&  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 5 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
Surprise~\cite{DBLP:journals/jossw/Hug20}    &  &  &  &  &  &  &  &  & \checkmark & \checkmark &  &  & \checkmark & \checkmark &  & \checkmark &  & \checkmark & 6 &  &  &  &  &  &  &  &  & 0  & \checkmark &  &  & \checkmark & \checkmark &  &  &  & 3 \\ 
Cornac~\cite{DBLP:journals/jmlr/SalahTL20}   &  &  &  &  &  &  &  & \checkmark & \checkmark &  &  &  &  &  &  & \checkmark &  & \checkmark & 4 & \checkmark &  &  & \checkmark & \checkmark &  &  &  & 3  & \checkmark &  &  & \checkmark & \checkmark & \checkmark &  &  & 4 \\ 
RecBole~\cite{DBLP:journals/corr/abs-2011-01731}  &  &  &  & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark &  &  &  &  &  & \checkmark & 8 &  &  &  &  &  &  &  &  & 0  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & 7 \\ 
DaisyRec~\cite{DBLP:conf/recsys/SunY00Q0G20}  &  &  & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark &  &  &  &  &  &  &  & \checkmark & 7 & \checkmark &  &  & \checkmark & \checkmark &  &  &  & 3  &  &  & \checkmark &  & \checkmark & \checkmark &  & \checkmark & 4 \\ 

% \midrule

\framework & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{13} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{8}  & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{8} \\ 

\bottomrule
\end{tabularx}
}
%}
\vspace{0.7em}

{
\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{0.245em}
\rowcolors{6}{white}{gray!15}
\begin{tabularx}{\textwidth}{X@{\hskip 0.7em}llllllllllllllllllllllllllllllllllllll@{\hskip 0.7em}r@{\hskip 0.7em}r}

\hlineB{2.5}
\myrowcolour \multicolumn{ 41}{c}{\textbf{RECOMMENDER MODELS}}
\\
\toprule
 & \multicolumn{ 39}{c}{\textbf{Common Models}}
\\
 \cmidrule(r){2-39}

 & \rotatebox{90}{MostPop} & \rotatebox{90}{Random} & \rotatebox{90}{ItemKNN} & \rotatebox{90}{UserKNN} & \rotatebox{90}{PureSVD} & \rotatebox{90}{FunkSVD} & \rotatebox{90}{SVD++} & \rotatebox{90}{SLIM} & \rotatebox{90}{MF} & \rotatebox{90}{WRMF} & \rotatebox{90}{FM} & \rotatebox{90}{NeuMF} & \rotatebox{90}{BPRMF} & \rotatebox{90}{DMF} & \rotatebox{90}{FISM} & \rotatebox{90}{NMF} & \rotatebox{90}{NFM} & \rotatebox{90}{SoREC} & \rotatebox{90}{DeepFM} & \rotatebox{90}{PMF} & \rotatebox{90}{AFM} & \rotatebox{90}{FFM} & \rotatebox{90}{WBPR} & \rotatebox{90}{DSSM} & \rotatebox{90}{VBPR} & \rotatebox{90}{ConvMF} & \rotatebox{90}{GMF} & \rotatebox{90}{Caser} & \rotatebox{90}{VAECF} & \rotatebox{90}{I-AutoRec} & \rotatebox{90}{U-AutoRec} & \rotatebox{90}{CDAE} & \rotatebox{90}{CML} & \rotatebox{90}{LogMF} & \rotatebox{90}{LDA} & \rotatebox{90}{SocialMF} & \rotatebox{90}{SlopeOne} & \rotatebox{90}{SoReg}  &
  \rotatebox{90}{\textbf{Others}} &
 \rotatebox{90}{\textbf{Tot.}}\\ \toprule
 
 
LensKit Java~\cite{DBLP:conf/recsys/EkstrandLKR11}  &  &  & \checkmark & \checkmark &  & \checkmark &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  & 0 & 5 \\

Mymedialite~\cite{DBLP:conf/recsys/GantnerRFS11} & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  & \checkmark & \checkmark &  & 6 & 18 \\

RankSys~\cite{DBLP:conf/sigir/Vargas14} & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  &  & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  &  &  & 0 & 8 \\

LibRec~\cite{DBLP:conf/um/GuoZSY15} & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  & \checkmark &  &  &  & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark & \checkmark & 30 & 55 \\

Implicit\footnote{\url{https://github.com/benfred/implicit}} &  &  & \checkmark & \checkmark &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  & 0 & 4 \\

OpenRec~\cite{DBLP:conf/wsdm/YangBGHE18} &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  & \checkmark &  &  &  &  & \checkmark &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  & 7 & 11 \\

RecQ~\cite{DBLP:conf/icdm/Yu0YLGW19} &  &  &  &  & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  &  &  & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & \checkmark & \checkmark & 6 & 13 \\

DeepRec~\cite{DBLP:conf/isca/GuptaHSWRWL0W20} &  &  &  &  &  &  &  &  & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark &  &  & \checkmark &  &  & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  &  &  & 5 & 20 \\

LensKit Python~\cite{DBLP:conf/cikm/Ekstrand20} & \checkmark &  & \checkmark & \checkmark &  & \checkmark &  &  & \checkmark &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0 & 6 \\

Surprise~\cite{DBLP:journals/jossw/Hug20} &  &  & \checkmark & \checkmark & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  & 1 & 7 \\ 

Cornac~\cite{DBLP:journals/jmlr/SalahTL20} & \checkmark &  & \checkmark & \checkmark & \checkmark &  &  &  & \checkmark &  &  & \checkmark &  &  &  & \checkmark &  & \checkmark &  & \checkmark &  &  & \checkmark &  & \checkmark & \checkmark & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  &  & 21 & 35 \\ 

RecBole~\cite{DBLP:journals/corr/abs-2011-01731} & \checkmark &  & \checkmark &  &  &  &  &  &  &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  & \checkmark &  &  &  & \checkmark & \checkmark &  &  & \checkmark &  &  &  &  &  &  & 50 & \textbf{65} \\ 

DaisyRec~\cite{DBLP:conf/recsys/SunY00Q0G20} & \checkmark &  & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  &  & \checkmark &  & \checkmark &  & \checkmark &  &  &  &  &  &  &  & \checkmark &  &  & \checkmark &  &  &  &  &  &  & 0 & 14 \\

\framework & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  &  & & \checkmark & 19 & 50 \\

\bottomrule
\end{tabularx}

}

\vspace{0.7em}

{
\setlength{\tabcolsep}{0.8em}
\renewcommand{\arraystretch}{0.9}
\rowcolors{7}{gray!15}{white}
\begin{tabularx}{\textwidth}{X@{\hskip 1.8em}rrlllllr@{\hskip 1.8em}ccr}

\hlineB{2.5}
\myrowcolour \multicolumn{ 12}{c}{\textbf{EVALUATION OF RECOMMENDATION PERFORMANCE}}
\\

\toprule
 & \multicolumn{8}{c}{\textbf{Metric Families}} & \multicolumn{3}{c}{\textbf{Statistical Tests}} \\ 
 \cmidrule(r){2-9}\cmidrule(l){10-12}
& Accuracy 
& Error
& Coverage 
& Novelty 
& Diversity 
& Bias 
& Fairness 
& \textbf{Tot.}
& Paired t-test 
& Wilcoxon
& \textbf{Tot.} \\ 

\toprule

LensKit Java~\cite{DBLP:conf/recsys/EkstrandLKR11}      & 2 & 2 & \multicolumn{1}{r}{1} &  & \multicolumn{1}{r}{1} &  &  & 6 &&&0\\
Mymedialite~\cite{DBLP:conf/recsys/GantnerRFS11}        & 6 & 2 &  &  &  &  &  & 8 && &0\\ 
RankSys~\cite{DBLP:conf/sigir/Vargas14}                 & 7 & & \multicolumn{1}{r}{\textbf{3}} & \multicolumn{1}{r}{\textbf{6}} & \multicolumn{1}{r}{\textbf{18}} &  &  & 34 && &0\\ 
LibRec~\cite{DBLP:conf/um/GuoZSY15}                         & 6 & \textbf{4} &  &  &  &  &  & 10 && &0\\ 
Implicit\footnote{\url{https://github.com/benfred/implicit}} & & &  &  &  &  &  & 0  &&&0\\ 
OpenRec~\cite{DBLP:conf/wsdm/YangBGHE18}                        & 4 & &  &  &  &  &  & 4 &&&0\\ 
RecQ~\cite{DBLP:conf/icdm/Yu0YLGW19}                            & 6 & 2 &  &  &  &  &  & 8 && &0\\ 
DeepRec~\cite{DBLP:conf/isca/GuptaHSWRWL0W20}               & 6 & 2 &  &  &  &  &  & 8 && &0\\ 
LensKit Python~\cite{DBLP:conf/cikm/Ekstrand20}                         & 4 & 2 &  &  &  &  &  & 6 && &0\\ 
Surprise~\cite{DBLP:journals/jossw/Hug20} & & \textbf{4} &  &  &  &  &  & 4 && &0\\ 
Cornac~\cite{DBLP:journals/jmlr/SalahTL20} & 8 & 3 &  &  &  &  &  & 11 && &0\\ 
RecBole~\cite{DBLP:journals/corr/abs-2011-01731} & 8 & 3 &  &  &  &  &  & 11 &&&0\\ 
DaisyRec~\cite{DBLP:conf/recsys/SunY00Q0G20} & 8 & &  &  &  &  &  & 8 &&&0\\ 
\framework & \textbf{11} & 3 & \multicolumn{1}{r}{\textbf{3}} & \multicolumn{1}{r}{2} & \multicolumn{1}{r}{3} & \multicolumn{1}{r}{\textbf{10}} & \multicolumn{1}{r}{\textbf{4}} & \textbf{36} & \checkmark & \checkmark &\textbf{2}\\ 
\bottomrule
\end{tabularx}

}

%\end{center}
\label{}
\end{table*}


==> tables/metrics.tex <==
\begin{table}[htbp]
\caption{}
\small
\begin{adjustbox}{width=\columnwidth,center}
\rowcolors{4}{gray!15}{white}
\begin{tabular}{l@{\hskip 1.5em}rrlllllr@{\hskip 1.5em}cc}
\toprule
 & \multicolumn{8}{c}{\textbf{METRICS}} & \multicolumn{2}{c}{\textbf{STATISTICAL TESTS}} \\ 
 \cmidrule(r){2-9}\cmidrule(l){10-11}
& \multicolumn{1}{l}{\textbf{Accuracy}} 
& \multicolumn{1}{l}{\textbf{Error}} 
& \textbf{Coverage} 
& \textbf{Novelty} 
& \textbf{Diversity} 
& \textbf{Bias} 
& \textbf{Fairness} 
& \multicolumn{1}{l}{\textbf{Total}}
& \textbf{Paired t-test} 
& \textbf{Wilcoxon} \\ 

\toprule

LensKit Java~\cite{DBLP:conf/recsys/EkstrandLKR11}      & 2 & 2 & \multicolumn{1}{r}{1} &  & \multicolumn{1}{r}{1} &  &  & 6 &&\\
Mymedialite~\cite{DBLP:conf/recsys/GantnerRFS11}        & 6 & 2 &  &  &  &  &  & 8 && \\ 
RankSys~\cite{DBLP:conf/sigir/Vargas14}                 & 7 & & \multicolumn{1}{r}{\textbf{3}} & \multicolumn{1}{r}{\textbf{6}} & \multicolumn{1}{r}{\textbf{18}} &  &  & 34 && \\ 
LibRec~\cite{DBLP:conf/um/GuoZSY15}                         & 6 & \textbf{4} &  &  &  &  &  & 10 && \\ 
Implicit\footnote{\url{https://github.com/benfred/implicit}} & & &  &  &  &  &  & 0  &&\\ 
OpenRec~\cite{DBLP:conf/wsdm/YangBGHE18}                        & 4 & &  &  &  &  &  & 4 &&\\ 
RecQ~\cite{DBLP:conf/icdm/Yu0YLGW19}                            & 6 & 2 &  &  &  &  &  & 8 && \\ 
DeepRec~\cite{DBLP:conf/isca/GuptaHSWRWL0W20}               & 6 & 2 &  &  &  &  &  & 8 && \\ 
LensKit Python~\cite{DBLP:conf/cikm/Ekstrand20}                         & 4 & 2 &  &  &  &  &  & 6 && \\ 
Surprise~\cite{DBLP:journals/jossw/Hug20} & & \textbf{4} &  &  &  &  &  & 4 && \\ 
Cornac~\cite{DBLP:journals/jmlr/SalahTL20} & 8 & 3 &  &  &  &  &  & 11 && \\ 
RecBole~\cite{DBLP:journals/corr/abs-2011-01731} & 8 & 3 &  &  &  &  &  & 11 &&\\ 
DaisyRec~\cite{DBLP:conf/recsys/SunY00Q0G20} & 8 & &  &  &  &  &  & 8 &&\\ 
\framework & \textbf{11} & 3 & \multicolumn{1}{r}{\textbf{3}} & \multicolumn{1}{r}{2} & \multicolumn{1}{r}{3} & \multicolumn{1}{r}{\textbf{10}} & \multicolumn{1}{r}{\textbf{4}} & \textbf{36} & \checkmark & \checkmark \\ 
\bottomrule
\end{tabular}
 \end{adjustbox}
\label{}
\end{table}

==> tables/models.tex <==
{
\setlength{\tabcolsep}{0.24em}
\begin{table*}[htbp]
\caption{}
\small
\rowcolors{4}{gray!15}{white}
\begin{tabular}{l@{\hskip 0.8em}llllllllllllllllllllllllllllllllllllll@{\hskip 0.8em}rr}

\toprule
 & \multicolumn{ 39}{c}{\textbf{COMMON MODELS}}
\\
 \cmidrule(r){2-39}

 & \rotatebox{90}{MostPop} & \rotatebox{90}{Random} & \rotatebox{90}{ItemKNN} & \rotatebox{90}{UserKNN} & \rotatebox{90}{PureSVD} & \rotatebox{90}{FunkSVD} & \rotatebox{90}{SVD++} & \rotatebox{90}{SLIM} & \rotatebox{90}{MF} & \rotatebox{90}{WRMF} & \rotatebox{90}{FM} & \rotatebox{90}{NeuMF} & \rotatebox{90}{BPRMF} & \rotatebox{90}{DMF} & \rotatebox{90}{FISM} & \rotatebox{90}{NMF} & \rotatebox{90}{NFM} & \rotatebox{90}{SoREC} & \rotatebox{90}{DeepFM} & \rotatebox{90}{PMF} & \rotatebox{90}{AFM} & \rotatebox{90}{FFM} & \rotatebox{90}{WBPR} & \rotatebox{90}{DSSM} & \rotatebox{90}{VBPR} & \rotatebox{90}{ConvMF} & \rotatebox{90}{GMF} & \rotatebox{90}{Caser} & \rotatebox{90}{VAECF} & \rotatebox{90}{I-AutoRec} & \rotatebox{90}{U-AutoRec} & \rotatebox{90}{CDAE} & \rotatebox{90}{CML} & \rotatebox{90}{LogMF} & \rotatebox{90}{LDA} & \rotatebox{90}{SocialMF} & \rotatebox{90}{SlopeOne} & \rotatebox{90}{SoReg}  &
  \rotatebox{90}{\textbf{Others}} &
 \rotatebox{90}{\textbf{Tot.}}\\ \toprule
 
 
LensKit Java~\cite{DBLP:conf/recsys/EkstrandLKR11}  &  &  & \checkmark & \checkmark &  & \checkmark &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  & 0 & 5 \\

Mymedialite~\cite{DBLP:conf/recsys/GantnerRFS11} & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  & \checkmark & \checkmark &  & 6 & 18 \\

RankSys~\cite{DBLP:conf/sigir/Vargas14} & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  &  & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  &  &  & 0 & 8 \\

LibRec~\cite{DBLP:conf/um/GuoZSY15} & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  & \checkmark &  &  &  & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark & \checkmark & 30 & 55 \\

Implicit\footnote{\url{https://github.com/benfred/implicit}} &  &  & \checkmark & \checkmark &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  & 0 & 4 \\

OpenRec~\cite{DBLP:conf/wsdm/YangBGHE18} &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  & \checkmark &  &  &  &  & \checkmark &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  & 7 & 11 \\

RecQ~\cite{DBLP:conf/icdm/Yu0YLGW19} &  &  &  &  & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  &  &  & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & \checkmark & \checkmark & 6 & 13 \\

DeepRec~\cite{DBLP:conf/isca/GuptaHSWRWL0W20} &  &  &  &  &  &  &  &  & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark &  &  & \checkmark &  &  & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  &  &  & 5 & 20 \\

LensKit Python~\cite{DBLP:conf/cikm/Ekstrand20} & \checkmark &  & \checkmark & \checkmark &  & \checkmark &  &  & \checkmark &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0 & 6 \\

Surprise~\cite{DBLP:journals/jossw/Hug20} &  &  & \checkmark & \checkmark & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark &  & 1 & 7 \\ 

Cornac~\cite{DBLP:journals/jmlr/SalahTL20} & \checkmark &  & \checkmark & \checkmark & \checkmark &  &  &  & \checkmark &  &  & \checkmark &  &  &  & \checkmark &  & \checkmark &  & \checkmark &  &  & \checkmark &  & \checkmark & \checkmark & \checkmark &  & \checkmark &  &  &  &  &  &  &  &  &  & 21 & 35 \\ 

RecBole~\cite{DBLP:journals/corr/abs-2011-01731} & \checkmark &  & \checkmark &  &  &  &  &  &  &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  & \checkmark &  &  &  & \checkmark & \checkmark &  &  & \checkmark &  &  &  &  &  &  & 50 & \textbf{65} \\ 

DaisyRec~\cite{DBLP:conf/recsys/SunY00Q0G20} & \checkmark &  & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  &  & \checkmark &  & \checkmark &  & \checkmark &  &  &  &  &  &  &  & \checkmark &  &  & \checkmark &  &  &  &  &  &  & 0 & 14 \\

\framework & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  &  & & \checkmark & 19 & 50 \\

\bottomrule
\end{tabular}
\label{}
\end{table*}
}

==> tables/strategies.tex <==
{
\setlength{\tabcolsep}{0.28em}
\begin{table*}[tbp]
\caption{Hold-out (HO), Cross-validation (CV)}
\small
\begin{center}
%\resizebox{\textwidth}{!}{%
\rowcolors{21}{gray!15}{white}
\begin{tabular}{l@{\hskip 0.8em}llllllllllllllllllr@{\hskip 0.8em}llllllllr@{\hskip 0.8em}llllllllr}

\toprule
 \multicolumn{ 38}{c}{\textbf{STRATEGIES}} \\

\toprule

 & \multicolumn{ 19}{c}{\textbf{Splitting}}
 & \multicolumn{ 9}{c}{\textbf{Filtering}}
 & \multicolumn{ 9}{c}{\multirow{1}{*}{\textbf{Hyperparam.} \textbf{tuning} }} 
\\
 \cmidrule(r){2-20}\cmidrule(lr){21-29}\cmidrule(l){30-38}


 & \multicolumn{ 7}{c}{\textbf{Temporal}} 
 & \multicolumn{ 10}{c}{\textbf{Random}} 
 & \multicolumn{ 1}{c}{\multirow{2}{*}{\textbf{Fix}}} 
 & \multicolumn{ 1}{c}{} 
 & \multicolumn{ 3}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{Rating} \\ \textbf{Thld.} \end{tabular}}} 
 & \multicolumn{ 5}{c}{\multirow{2}{*}{\textbf{$k$-core}}} 
 & \multicolumn{1}{l}{} 
 & \multicolumn{ 4}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{Search} \\\textbf{Strategy}\end{tabular}}}
 & \multicolumn{ 4}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{Search} \\\textbf{Space}\end{tabular}}}
  & \multicolumn{1}{l}{}
 \\
 \cmidrule(r){2-8}\cmidrule(lr){9-18}

 
 & \multicolumn{ 2}{c}{Fix} 
 & \multicolumn{ 5}{c}{HO} 
 & \multicolumn{ 5}{c}{HO} 
 & \multicolumn{ 3}{c}{$K$-HO} 
 & \multicolumn{ 2}{c}{CV} 
 & \multicolumn{ 1}{l}{} 
 & \multicolumn{ 1}{l}{} 
 & \multicolumn{ 3}{l}{} 
 & \multicolumn{ 5}{l}{} 
%  & \multicolumn{1}{l}{} 
%  & \multicolumn{ 4}{c}{Search Strategy}
%  & \multicolumn{ 4}{c}{Search Space} 
%  & \multicolumn{1}{l}{} 
 \\ 
  \cmidrule(r){2-3}\cmidrule(lr){4-8}\cmidrule(lr){9-13} \cmidrule(lr){14-16}\cmidrule(lr){17-18} \cmidrule{19-19} 
  \cmidrule(r){21-23}  \cmidrule(l){24-28}    \cmidrule(r){30-33} \cmidrule(l){34-37}

 
 & \rotatebox{90}{Last} 
 & \rotatebox{90}{Hand}
 & \rotatebox{90}{By-Ratio Sys.}
 & \rotatebox{90}{By-Ratio User}
 & \rotatebox{90}{Leave-$1$-out}
 & \rotatebox{90}{Leave-$n$-in}
 & \rotatebox{90}{Leave-$n$-out}
 & \rotatebox{90}{By-Ratio Sys.}
 & \rotatebox{90}{By-Ratio User}
 & \rotatebox{90}{Leave-$1$-out}
 & \rotatebox{90}{Leave-$n$-in}
 & \rotatebox{90}{Leave-$n$-out}
 & \rotatebox{90}{By-Ratio Sys.}
 & \rotatebox{90}{Leave-$1$-out}
 & \rotatebox{90}{Leave-$n$-out}
 & \rotatebox{90}{$k$-folds Sys.}
 & \rotatebox{90}{$k$-folds User}
 & \multicolumn{1}{c}{\rotatebox{90}{Computed}}
 & \rotatebox{90}{\textbf{Tot.}} 
 
 & \rotatebox{90}{Numerical}
 & \rotatebox{90}{Distributional}
 & \rotatebox{90}{User-Based}
%   & \rotatebox{90}{$k\text{-core}_\textit{User}$}
%  & \rotatebox{90}{$k\text{-core}_\textit{Item}$}
%  & \rotatebox{90}{Iterative $k$-core}
%  & \rotatebox{90}{$n$ rounds $k$-core}
  & \rotatebox{90}{User}
 & \rotatebox{90}{Item}
 & \rotatebox{90}{Iterative}
 & \rotatebox{90}{$n$-rounds}
 & \multicolumn{1}{c}{\rotatebox{90}{cold users}}
 
 & \rotatebox{90}{\textbf{Tot.}}
 & \rotatebox{90}{Grid}
 & \rotatebox{90}{Annealing}
 & \rotatebox{90}{Bayesian} 
 & \rotatebox{90}{Random}
 & \rotatebox{90}{Choice}
 & \rotatebox{90}{Uniform}
 & \rotatebox{90}{Normal}
 & \multicolumn{1}{c}{\rotatebox{90}{Log-Uniform}}
 & \rotatebox{90}{\textbf{Tot.}}
 
\\ 
\toprule


LensKit Java~\cite{DBLP:conf/recsys/EkstrandLKR11}    &  &  &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  &  & \checkmark & \checkmark & 10 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
Mymedialite~\cite{DBLP:conf/recsys/GantnerRFS11}   &  &  & \checkmark & \checkmark &  &  & \checkmark & \checkmark &  &  &  &  &  &  &  & \checkmark &  & \checkmark & 6 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
RankSys~\cite{DBLP:conf/sigir/Vargas14}       &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & 1 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
LibRec~\cite{DBLP:conf/um/GuoZSY15}         &  &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  & \checkmark &  & \checkmark &  & \checkmark & 11 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
Implicit\footnote{\url{https://github.com/benfred/implicit}}    &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & 1 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
OpenRec~\cite{DBLP:conf/wsdm/YangBGHE18}        &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & 1 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
RecQ~\cite{DBLP:conf/icdm/Yu0YLGW19} &  &  &  &  &  &  &  &  & \checkmark &  &  &  & \checkmark &  &  &  &  & \checkmark & 3 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
DeepRec~\cite{DBLP:conf/isca/GuptaHSWRWL0W20} &  &  &  &  &  &  &  & \checkmark &  &  &  &  &  &  &  &  &  & \checkmark & 2 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
LensKit Python~\cite{DBLP:conf/cikm/Ekstrand20}&  &  &  &  &  &  &  &  &  &  &  &  &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 5 &  &  &  &  &  &  &  &  & 0  &  &  &  &  &  &  &  &  & 0 \\ 
Surprise~\cite{DBLP:journals/jossw/Hug20}    &  &  &  &  &  &  &  &  & \checkmark & \checkmark &  &  & \checkmark & \checkmark &  & \checkmark &  & \checkmark & 6 &  &  &  &  &  &  &  &  & 0  & \checkmark &  &  & \checkmark & \checkmark &  &  &  & 3 \\ 
Cornac~\cite{DBLP:journals/jmlr/SalahTL20}   &  &  &  &  &  &  &  & \checkmark & \checkmark &  &  &  &  &  &  & \checkmark &  & \checkmark & 4 & \checkmark &  &  & \checkmark & \checkmark &  &  &  & 3  & \checkmark &  &  & \checkmark & \checkmark & \checkmark &  &  & 4 \\ 
RecBole~\cite{DBLP:journals/corr/abs-2011-01731}  &  &  &  & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark &  &  &  &  &  & \checkmark & 8 &  &  &  &  &  &  &  &  & 0  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & 7 \\ 
DaisyRec~\cite{DBLP:conf/recsys/SunY00Q0G20}  &  &  & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark &  &  &  &  &  &  &  & \checkmark & 7 & \checkmark &  &  & \checkmark & \checkmark &  &  &  & 3  &  &  & \checkmark &  & \checkmark & \checkmark &  & \checkmark & 4 \\ 

% \midrule

\framework & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{13} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{8}  & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{8} \\ 

\bottomrule
\end{tabular}
%}
\end{center}
\label{}
\end{table*}
}
